Risk-Calibrated Human-Robot Interaction via Set-Valued Intent Prediction

Tasks where robots must anticipate human intent, such as navigating around a cluttered home or sorting everyday items, are challenging because they exhibit a wide range of valid actions that lead to similar outcomes. Moreover, zero-shot cooperation between human-robot partners is an especially challenging problem because it requires the robot to infer and adapt on the fly to a latent human intent, which could vary significantly from human to human. Recently, deep learned motion prediction models have shown promising results in predicting human intent but are prone to being confidently incorrect. In this work, we present Risk-Calibrated Interactive Planning (RCIP), which is a framework for measuring and calibrating risk associated with uncertain action selection in human-robot cooperation, with the fundamental idea that the robot should ask for human clarification when the risk associated with the uncertainty in the human's intent cannot be controlled. RCIP builds on the theory of set-valued risk calibration to provide a finite-sample statistical guarantee on the cumulative loss incurred by the robot while minimizing the cost of human clarification in complex multi-step settings. Our main insight is to frame the risk control problem as a sequence-level multi-hypothesis testing problem, allowing efficient calibration using a low-dimensional parameter that controls a pre-trained risk-aware policy. Experiments across a variety of simulated and real-world environments demonstrate RCIP's ability to predict and adapt to a diverse set of dynamic human intents.

==> rebuttal/statement_of_changes.tex <==


\onecolumn

\section*{Our Meta Comments}
We sincerely thank the reviewers and the Area Chair for their detailed feedback. We are happy to see that the reviewers appreciated (1) the strong motivation for leveraging statistical risk calibration for controlling both planning success rates and human help rates in HRI, (2) the intuitive theoretical approach of the framework, and (3) the effective application in several settings in both simulation and hardware. In response to the reviewers’ concerns and suggestions, we have made appropriate changes to the paper and performed new experiments as summarized below. We address the main concerns first, and we then respond to individual reviewers. For convenience, we have attached the revised manuscript to this document, with changes highlighted in \rebuttal{blue color}.

\vspace{0.2cm}
\section*{Summary of Major Changes}
\noindent 
\textbf{Changes addressing paper writing, paper quality:}
\begin{enumerate}
    \item We have thoroughly revised the paper to improve the overall quality of exposition, and to eliminate typos and repeated sentences. 
    \item We have substantially revised Figures \hyperlink{page.1}{1} and \ref{fig:pipeline} to make the overall RCIP procedure more clear. 
    \item We have revised Figures \ref{fig: hallway} and \ref{fig: habitat_bimanual} and additionally add several plots to Figure \ref{fig: baselines} to help clarify the experimental settings. 
\end{enumerate}
\textbf{Changes addressing the provision of key details of methods and experiments:}
\begin{enumerate}
    \item We have provided more detail in the Experiments section, and we now provide an extensive description of each environment and the source of intent ambiguity. 
\end{enumerate}
\textbf{Changes addressing the functional form of the intent prediction model:}
\begin{enumerate}
    \item We have added a more extensive description of $g_\theta$ in Section \ref{formulation}. We have added equation \eqref{eqn: intent_softmax}, which defines the model’s heuristic confidence as a softmax function over the intent space. 
    \item We have added a verbal description of the specific form of $g_\theta$ for each experiment in Section \ref{Experiments} (Experiments) and in Appendix \ref{Appendix: Models}.
\end{enumerate}
 \textbf{Changes addressing the concern on handling more complex interactive scenarios:}
\begin{enumerate}
    \item We ran an additional hardware experiment in a bimanual manipulation task requiring human-to-robot object transfer and a larger number of intents (>30). We have added these new results to Section \ref{Experiments} (Experiments).
    \item We added Figure \ref{fig: habitat_bimanual} (left) to illustrate the multi-step application of RCIP in Habitat Social Navigation. We have also added an illustration of single-step RCIP applied to Bimanual Sorting (right). 
\end{enumerate}
\textbf{Changes addressing the similar performance to KnowNo \cite{ren2023robots} and Simple Set baselines:}
\begin{enumerate}
    \item We reran our experiments, this time focusing closely on the choice of temperature range (one of our tunable model parameters $\theta$) for the softmax scoring of each intent. When changing our temperature range to a log scale, we notice almost uniform improvement over KnowNo, now achieving up to an $87\%$ reduction in the planning help rate. We have updated Figure \ref{fig: baselines} to reflect this change – it now includes help rate curves for all environments. The improvement against Simple Set is even more pronounced (see, e.g., the updated Figure \ref{fig: baselines}).
    \item We have updated the comparison to baselines at target success levels in all settings – please see Tables \ref{tab: hallway}-\ref{tab: bimanual}.
    \item We have added Appendix \ref{Appendix: discussion} to additionally discuss (1) why temperature optimization can lead to significant improvements over naive initialization in set-valued prediction, and (2) the potential pitfalls of planning using open-ended language, as is used in the original procedure proposed by KnowNo. 
\end{enumerate}
\textbf{Changes addressing the initial accuracy of prediction model on the effectiveness of the framework:}
\begin{enumerate}
    \item We have added Table \ref{tab: hallway_earlystopping} showing the help rate required to achieve $85\%$ action coverage in the Hallway navigation setting for three checkpoints over the prediction model’s training. Overall, a more well-trained model requires less help. 
\end{enumerate}
\textbf{Changes involving the realism of the human interaction in the experiments:}
\begin{enumerate}
    \item We have added more detail in the Appendix (Sections \ref{Appendix: experiments}-\ref{Appendix: implementation}) on the separation between the predictor training, intent-conditioned policy training, and sampling from the intent distribution during calibration and use of human feedback. 
\end{enumerate}



\vspace{0.2cm}
\section*{Area Chair’s Comments}

\noindent
\emph{The strengths include the relevance of the problem, the intuitive theoretical idea, and the demonstrated effectiveness in various environments. The writing quality of the paper needs to be significantly improved. Key details of method and experiments need to be provided.}
% \textbf{Concern on the mathematical accessibility of the paper and use of jargon.}
\begin{itemize}
    \item We thank the Area Chair for acknowledging the relevance of the problem, and our contributions in both theory and applications of the framework. We have significantly revised the paper to clarify the exposition. We have updated nearly every figure (Figures \hyperlink{page.1}{1}-\ref{fig: baselines}) and Table (Tables \ref{tab: hallway}-\ref{tab: bimanual}) to provide additional context and new results. We now also provide an appendix to provide additional details and discussion. We hope that these changes will help clarify the main story. 
\end{itemize}

\section*{Addressing the Main Concerns}
\textbf{Concern on the generalization of the framework to more complex scenarios with many intents.}
\begin{itemize}
    \item We would like to clarify that our experiment scenarios are already quite extensive, covering different types and quantities of intent. Our Habitat simulation environment consists of 77 objects from the YCB dataset \cite{calli2015ycb}, up to 10 of which are randomly sampled per scene. Scenes are randomly sampled from the  Habitat Synthetic Scenes Dataset  \cite{khanna2023habitat}, which is a dataset of 211 high-quality 3D scenes containing over 18k individual models of real-world objects. In our open-category sorting setup in hardware, our object set consists of 200 semantically similar objects (now shown in Appendix \ref{Appendix: experiments}), with up to 15 objects per category. 
    \item Since the original submission, we have added an additional experiment for a bimanual setup where the robot must sort an object for the human. In this experiment, the intent space is the combination of bins that the human finds acceptable for sorting, and there are over 30 possible combinations. Using our setup, RCIP achieves a target success rate of $75\%$ using $85\%$ help versus $93\%$ for KnowNo. 
\end{itemize}
\textbf{Concern on the quality of the intent predictor.}
\begin{itemize}
    \item We acknowledge that the performance of our framework scales with the difficulty of intent prediction capabilities of intent predictors. In general, scenarios where intents are challenging to predict less performant predictors will require more help. To this end, here we address how RCIP can be used to extract the best possible performance out of available predictors in spite of miscalibration.
    \item Since the submission, we re-ran our experiments with a wider set of softmax temperatures (the softmax scores are now defined in Eqn \eqref{eqn: intent_softmax}). We re-ran our experiments with a log-scale temperature and found that the help rate reduction improves to $8-87\%$ from the $5-30\%$ achieved using the original risk calibration results. Temperature scaling has been used extensively in other prediction literature (see, e.g., \cite{platt1999probabilistic, guo2017calibration, xi2024does}) for achieving calibration, but usually requires manual search or fine-tuning. Instead, RCIP offers a theoretically principled algorithm for automating the search for an optimal temperature by focusing on its effect on downstream risk. Additionally, we now use the (recently released) official GPT-4V model for the Open-Category Sorting and Bimanual Sorting experiments. We have updated the descriptions of the experiments to reflect this change. 
    \item We have added an additional experiment in Table \ref{tab: hallway_earlystopping} that shows help rates needed in Hallway Navigation at a target success level of $85\%$ for three predictors of varying quality. The No-Help success rates for the predictors are $59\%$, $68\%$, and $100\%$ (a completely converged model). We use RCIP to calibrate the prediction threshold and temperature needed to achieve the target success level with minimal help for each model. The resultant help rates are $27\%$, $4\%$, and $0\%$ respectively. In summary, RCIP allows the end-user to achieve more fine-grained control over the success rate of the predictor with human help, but the procedure also benefits from having a better prediction model. 
\end{itemize}
\textbf{Concern on simulated humans.}
\begin{itemize}
    \item While the hallway and social navigation experiments use a simulated human, the open-category sorting experiments (included in the original submission) and the bimanual manipulation experiments (newly added) both use real human intents with zero-shot inference with GPT-4V. Specifically, the human is asked to choose, given an object (see Appendix \ref{Appendix: experiments} for the full set)  and a set of bins full of context objects, the correct placement for the object. The human’s chosen bin(s) are stored at each timestep and used to compute an intent-conditioned action.
\end{itemize}
\textbf{Concern on quantitative results and similar performance to KnowNo.}
The conformal prediction approach used by KnowNo ensures a minimal average prediction set size subject to a given coverage guarantee \cite{sadinle2019least}. Therefore, the risk control procedure used in RCIP may in fact produce similar results to conformal prediction methods for some fixed model parameters (for example, when the model temperature is close to the optimal value). However, our approach differs in two key ways:
\begin{itemize}
    \item RCIP can be used to provide direct bounds on the human help rate using the procedure detailed in Section \ref{section: approach}. Thus, RCIP provides a guarantee on the numerical value of the help rate whereas KnowNo does not. 
    \item When the default temperature is not close to the optimal value, the improvements from RCIP can be significant. Since RCIP tests multiple risk hypotheses simultaneously,our method automates temperature calibration without the need for a separate calibration dataset. Since the original submission, we have verified that optimal temperature selection can increase the improvement over KnowNo from $30\%$ to $87\%$. 
\end{itemize}




 

\vspace{0.2cm}
\section*{Reviewer rDNr’s Comments}

We thank Reviewer rDNr for their support and constructive feedback. In particular, we appreciate the concerns regarding the necessity for conditional determinism of the agents' actions, the accuracy of the intent prediction model, and the tracking of the intent-conditioned policy. 

\vspace{0.25cm}
\noindent
\textbf{Concern on conditional determinism of human’s intent-conditioned action:}
\begin{itemize}
    \item Thank you for pointing this out. We originally included this assumption to simplify the dynamic program formulation in equations \eqref{eqn: value_function} and \eqref{eqn: action_value_function}. In fact, this assumption is not necessary. If the human’s intent is known, the robot can always plan an intent-conditioned policy whether the human’s action is stochastic or not. Therefore, we have removed the assumption. The RCIP intent-conditioned policies do not need to be deterministic, just consistent with the human intent. 
\end{itemize}

\vspace{0.25cm}
\noindent
\textbf{Concern on inaccuracy of predicted intents:}
\begin{itemize}
    \item The predicted intent scores can indeed be inaccurate; however, the RCIP framework (namely, risk calibration and asking for help) ensures that the robot obtains a calibrated task success rate in spite of the incorrect predictions. For all experiments, we show a comparison between RCIP and a “no help” baseline,  which uses the raw intent prediction. In most settings, the “no help” baseline attains a success rate of between $40-60\%$, while our method achieves the target plan success rate, set at $85\%$ for the Hallway and Social Navigation settings and $75\%$ for the zero-shot sorting and bimanual settings.  
    \item To further clarify this point, we have provided an additional table: Table \ref{tab: hallway_earlystopping}. We checkpoint the intent prediction model throughout training to emulate a poorly trained prediction model. Since our method permits predicting a set of intents that the human can reduce to a singleton through help, we can guarantee that the true human intent is included (up to some probability). At various levels of training, our method is able to maintain a consistent miscoverage level, but with more help needed for less performant models. We see the ability of our method to provide guaranteed bounds on risk despite inaccuracies in the predicted intent as a significant strength.
\end{itemize}
\vspace{0.25cm}
\noindent
\textbf{Concern on perfect action tracking:}
\begin{itemize}
    \item We are not sure what is meant by tracking the planned actions. The intent-conditioned robot policy does not need to be optimal. As long as the robot policy is consistent with the human intent, the risk calibration procedure is feasible. If action tracking is a concern (e.g., social navigation in a narrow hallway), RCIP allows the end user to specify other notions of risk, e.g. collision rates, in the calibration procedure.
\end{itemize}

\vspace{0.2cm}
\section*{Reviewer xPPZ’s Comments}
We thank Reviewer xPPZ for their thorough and very constructive feedback. In particular, we appreciate their questions regarding the scenario distribution and prediction models for the various environments. We furthermore appreciate their concerns regarding similar performance to the KnowNo and Simple Set baselines and suggestions for imporvment of Figures \ref{fig:pipeline}-\ref{fig: habitat_bimanual}.

\vspace{0.2cm}
\noindent
\textbf{Concern on level of detail for scenario distributions and calibration dataset.}
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item Thank you for the feedback. We have added the critical details in the Experiments section, and we have added some more granular detail in the Appendix. We added detail in Appendix \ref{Appendix: experiments} on the set of intents and sources of intent ambiguity for each experiment, and we define the scenario distribution for each setting, including how we sample from it.    
\end{itemize}

\vspace{0.25cm}
\noindent
\textbf{Concern on specific form of the prediction model for various environments.}
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item We have similarly added the critical details in the Section \ref{Experiments} (Experiments). We added details in Appendix \ref{Appendix: Models} on the architecture of the predictor, training procedure for the hand-crafted intent predictors (Hallway and Social Navigation) and intent-conditioned policy (Hallway). We also describe in more detail the intent prediction process for Open-Category Sorting and Bimanual Sorting using GPT-4V. 
\end{itemize}

\vspace{0.25cm}
\noindent
\textbf{Concern on the clarity of Figure \ref{fig:pipeline}.}
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item Thank you for the suggestion. We have revised Figure \ref{fig:pipeline} to clarify the risk calibration aspect of RCIP, with special attention to the inputs and outputs for each column. We hope that the revised figure conveys a more intuitive understanding of the RCIP process. 
\end{itemize}

\vspace{0.25cm}
\noindent
\textbf{Concern on similarity to KnowNo and Simple Set baselines.}
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item We re-ran our experiments with a larger range of temperatures (a scalar weighting to the predictor’s log probabilities before the softmax operation) and found that with this increased range, the improvement over KnowNo increases from $5-30\%$ to $8-87\%$. We have added more help rate curves in Figure \ref{fig: baselines} to illustrate this difference. These results demonstrate the significant improvements afforded by the ability to tune model parameters (e.g., temperature scaling), which RCIP allows us to do in a principled manner.
\end{itemize}
\vspace{0.25cm}
\noindent
\textbf{Concern on generalization to more complex environments. }
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item To showcase the performance of RCIP in more complex cooperation settings, we have provided an additional hardware experiment in a complex bimanual manipulation setting. Specifically, the robot is asked to help a human sort a set of objects when there is significant ambiguity in which bin the object should be sorted. This intent set is the power set of the five bins on the table, so there are 31 intents possible (bin 1, bin 2, bin3, bin 4, bin 5, bins 1 or 2, bins 1 or 3, …) when excluding the empty set. We showcase RCIP’s improvement against KnowNo when there is a larger number of intents. At a target success level of $75\%$, RCIP requires $85\%$ help versus $93\%$ for KnowNo and $95\%$ for Simple Set (lower is better).  We also show in Appendix \ref{Appendix: discussion} that KnowNo, which describes plans in open-ended language, may fail to succinctly characterize the human’s intent, resulting in unpredictably diverse plans that must be parsed by a low-level language-conditioned policy, such as RT-2 \cite{brohan2023rt}.
\end{itemize}
\vspace{0.25cm}
\noindent
\textbf{Concern on Figures \ref{fig: hallway} and \ref{fig: habitat_bimanual}.}
% \textbf{Concern on computational complexity:}
\begin{itemize}
    \item Thank you for the suggestion. We have significantly revised the figures in the Section \ref{Experiments} (Experiments).  Figure \ref{fig: hallway} has been cut to a single frame with overlaid trajectories, to show the diversity in human intent. Some example rollouts have been moved to the appendix. Figure \ref{fig: habitat_bimanual} has been changed to show a rollout of RCIP in the multi-step setting in Social Navigation. Additionally, Figure \ref{fig: habitat_bimanual} shows a bimanual sorting, an additional experiment we added to showcase RCIP’s performance when the intent space is large (about 30 intents).
\end{itemize}





\vspace{0.2cm}
\section*{Reviewer g2Mt’s Comments}
We thank Reviewer g2Mt for their constructive and supportive comments to our manuscript. We appreciate that you think our idea is intuitive and reasonable, and that the method is generally applicable as shown in the initial experiments. We acknowledge the clarity of the previous submission was limited by some inconsistent notation, which we have addressed in the revised version.

\vspace{0.25cm}
\noindent
\textbf{Concern on notational clarity.}

Thank you for the feedback. We have fixed or eliminated the minor typos. In addition, we have made the following changes:
\begin{itemize}
    \item$\theta$ is now referred to as a “tunable parameter” to avoid confusion.
    \item We have changed ``intent'' to ``intent dynamics'' to Section \ref{formulation}-C and elsewhere in the paper.
    \item We have added the superscript in Eq. \eqref{eqn: intent_softmax} and provided a running example with Figure \hyperlink{page.1}{1} in a new remark. 
    \item We have clarified these points in the main text. To streamline the presentation, we have dropped the ``policy set'' and present the robot’s overall policy during deployment as the prediction-to-action distillation process. 
    \item We have defined the $[T]$ notation.
\end{itemize}


\vspace{0.25cm}
\noindent
\textbf{Concern on the general form of $g_\theta$ and specific form for each environment.}
\begin{itemize}
    \item The function $g_\theta$ outputs softmax scores over the possible human intents. Therefore, $g_\theta$ is a function that maps the context $x$ to a vector of real-number softmax scores. We have added Eqn. \eqref{eqn: intent_softmax} to make this functional form explicit. In general, $g_\theta$ can be any function, as long as it satisfies the definition above. In practice, we use a neural network (either a hand-crafted transformer prediction network, or a foundation model). We use the temperature to re-weight the softmax scores. This re-weighting is independent of the implementation of $g_\theta$. We have clarified the specific implementation of $g_\theta$ for all examples in the Experiments section and in the Appendix. 
\end{itemize}

\vspace{0.25cm}
\noindent
\textbf{Concern on modeling the human.}
\begin{itemize}
    \item The human is simulated for the hallway and habitat experiments. For the open-category sorting and (new) bimanual experiment, we have a human in the loop. The human is asked to provide their true intent at each timestep given the context (for example, picking which bin they would choose to sort the object). Regardless of the training data used to train the intent predictor, this allows us to calibrate the predictor’s performance for a particular human. However, poorly performing predictors will require more help on behalf of the human. We have clarified this in the text and provided a small experiment in Table II to showcase what happens to the help rate when the intent prediction model is under-trained.
\end{itemize}


\twocolumn
\newpage



==> subtex/extensions.tex <==
\subsection{Shruti: End-to-End Risk Calibration on Hardware}

Suppose we are now interested in the case where there are multiple acceptable intents per time step, i.e. multiple robot actions are acceptable. Now, the robot has a ``choice'' in which action it executes. Let $Z$ be the set of the multiple acceptable human intents. 

Let $\mathcal D$ be an unknown distribution over i.i.d. scenarios such that $\xi \sim \mathcal D$. Let $s$ serve as an additional label such that if $s=1$, then the policy succeeds; otherwise, the policy fails. If we fix a policy for the human and the robot and assume that the robot has ground-truth knowledge of z, then the distribution over scenarios induces a distribution over the context-label $(\bar{x}, z)$, where the context  contains a history of the previous states up to and including the current state at time $t$. Assume that the policy success $s$ is drawn from a distribution $E$. Assume we are given an augmented calibration set  $\mathcal C_A = \{(\bar x_i, C_i, s_i)\}_{i=1}^M \sim D \times E$, where $Z = \{z_{i}^j\}_{j=1}^{N_i}$ contains the set of acceptable options. We seek to define a measurable function $\beta(\bar x, Z, i)$ that samples an action from the set of correct actions to maximize the action success rate. 

Possible assumptions.
\begin{enumerate}
    \item There's at least one action that will succeed (but we don't know which one it is)
    \item The robot can always ask for help, and have the human complete the action instead 
    \item Can we take the intersection with the set of robot's possible actions? 
\end{enumerate}

==> subtex/hardware.tex <==
\section{Hardware}


